Perfectly Clustering Words and Iterated Palindromes over a Ternary Alphabet

Recently, a new characterization of Lyndon words that are also perfectly clustering was proposed by Lapointe and Reutenauer (2024). A word over a ternary alphabet {a,b,c} is called perfectly clustering Lyndon if and only if it is the product of two palindromes and it can be written as apbqc where p and q are palindromes. We study the properties of palindromes appearing as factors p and q and their links with iterated palindromes over a ternary alphabet.

==> eptcsdata.tex <==
\providecommand{\firstpage}{134}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2024\\
EPTCS 403, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.403.28}{10.4204/EPTCS.403.28}}

